$P_1$--Nonconforming Quadrilateral Finite Element Space with Periodic Boundary Conditions: Part II. Application to the Nonconforming Heterogeneous Multiscale Method

A homogenization approach is one of effective strategies to solve multiscale elliptic problems approximately. The finite element heterogeneous multiscale method (FEHMM) which is based on the finite element makes possible to simulate such process numerically. In this paper we introduce a FEHMM scheme for multiscale elliptic problems based on nonconforming spaces. In particular we use the noconforming element with the periodic boundary condition introduced in the companion paper. Theoretical analysis derives a priori error estimates in the standard Sobolev norms. Several numerical results which confirm our analysis are provided.

==> macros.tex <==
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}

\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\lemrefs}[2]{Lemmas~\ref{#1} and ~\ref{#2}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\proprefs}[2]{Propositions~\ref{#1} and ~\ref{#2}}
\newcommand{\rmkref}[1]{Remark~\ref{#1}}
\newcommand{\assref}[1]{Assumption~\ref{#1}}
\newcommand{\exrefs}[2]{Examples~\ref{#1} and ~\ref{#2}}
\newcommand{\exref}[1]{Example~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\figrefs}[2]{Figures~\ref{#1} and ~\ref{#2}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\tabrefs}[2]{Tables~\ref{#1} and ~\ref{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Up to here Added by Sheen
\newcommand\uwtil[1]{\underset{\widetilde{}}{#1}}
\newcommand\dutil[1]{\underset{\approx}{#1}}
\def\util{\uwtil}
\def\uta{\util a}
\def\utq{\util q}
\def\utz{\util z}

\newcommand{\eq}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\qe}{\end{eqnarray}}
\newcommand{\dd}{\textrm{d}}
\newcommand{\ii}{\textrm{i}}
\newcommand{\nn}{\nonumber}
\newcommand{\rb}[1]{\raisebox{1.5ex}[0pt]{#1}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\bal}{\begin{aligned}}
\newcommand{\eal}{\end{aligned}}
\newcommand{\bes}{\begin{eqnarray*}}
\newcommand{\ees}{\end{eqnarray*}}
\newcommand{\bs}{\begin{subeqnarray}}
\newcommand{\es}{\end{subeqnarray}}
\newcommand{\bss}{\begin{subeqnarray*}}
\newcommand{\ess}{\end{subeqnarray*}}
\newcommand{\tb}[1]{|\hskip -.08em|\hskip-.08em|#1|\hskip-.08em|\hskip-.08em|}

\newcounter{saveeqn}
\newcommand{\subeqn}{\setcounter{saveeqn}{\value{equation}}%
 \stepcounter{saveeqn}\setcounter{equation}{0}%
 \renewcommand{\theequation}{\mbox{\arabic{section}.\arabic{saveeqn}\alph
{equation}}}} %\alph, \roman
\newcommand{\reseteqn}{\setcounter{equation}{\value{saveeqn}}%
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}}
\newcommand{\BVP}{boundary value problem}
\newcommand{\PDE}{partial differential equation}
\newcommand{\PDEs}{partial differential equations}
\newcommand{\NIProlong}[1]{\mbox{${\cal NIP}_{#1}$}}
\newcommand{\NIProlongT}[1]{\mbox{${\cal NIP}_{#1}^T$}}
\newcommand{\Prolong}[1]{\mbox{${\cal P}_{#1}$}}
\newcommand{\ProlongT}[1]{\mbox{${\cal P}_{#1}^T$}}
\newcommand{\Restrict}[1]{\mbox{${\cal R}_{#1}$}}
\newcommand{\RestrictT}[1]{\mbox{${\cal R}_{#1}^T$}}
\newcommand{\RestrictA}[1]{\mbox{${\cal Q}_{#1}$}}
\newcommand{\RestrictFAS}[1]{\mbox{${\cal R}_{#1}^{(FAS)}$}}
\newcommand{\SolnSpace}[1]{\mbox{${\cal M}_{#1}$}}

\def\hat{\widehat}
\def\hQ{\widehat Q}
\def\hm{\widehat m}
\def\hx{\widehat x}
\def\hy{\widehat y}
\def\hz{\widehat z}
\def\hF{\widehat F}
\def\diam{\operatorname{diam}}
\def\supp{\operatorname{supp}}
\def\Span{\operatorname{Span}}
\def\mcE{\mathcal E}
\def\mcF{\mathcal F}
\def\Oh{\mathcal O}
\def\sL{\mathcal L}
\def\cC{\mathcal C}
\def\check{{\mathcal C}^h}
\def\globalcheck{p_{gc}^h}
\def\Pch{{\mathcal P}_{c}^h}
\def\Pcf{{\mathcal P}_{cf}^h}
\def\Pchp{{\mathcal P}_{c'}^h}
\def\Pcfp{{\mathcal P}_{cf'}^h}
\def\hf{\widehat f}
\def\hg{\widehat g}
\def\ha{\widehat a}
\def\hu{\widehat u}
\def\hv{\widehat v}
\def\hV{\widehat V}
\def\tw{\widetilde w}
\def\tilu{\widetilde u}
\def\z{\zeta}
\def\mbbR{\mathbb R}
\def\mbbC{\mathbb C}
\def\tt{T}
\def\tu{U}
\def\p{\partial}
\def\dt{\overline\partial}
\def\dsum{\displaystyle\sum}
\def\la{\lambda}
\def\ka{\kappa}
\def\Si{\Sigma}
\def\s{\sigma}
\def\O{\Omega}
\def\V{\mathcal V}
\def\Z{\mathcal Z}
\def\NC{\mathcal NC}
\def\NChz{{\mathcal NC}^h_0}
\def\NChz2d{{[\mathcal{NC}}^h_0]^2}
\def\tNChz2d{\widetilde {[\mathcal{NC}}^h_0]^2}
\def\oa{\overline{a}}
\def\ou{\overline{u}}
\def\bp{\overline{p}_h}
\def\tp{\widetilde{p}_h}
\def\bq{\overline{q}_h}
\def\tq{\widetilde{q}_h}
\def\bchi{\overline{\chi}_h}
\def\tchi{\widetilde{\chi}_h}
\def\o{\omega}
\def\ep{\epsilon}
\def\vep{\varepsilon}
\def\fy{\varphi}
\def\al{\alpha}
\def\de{\delta}
\def\De{\Delta}
\def\th{\theta}
\def\gk{{\Gamma_{\al,k}}}
\def\g{\gamma}
\def\G{\Gamma}
\def\as{\quad\text{as}\ }
\def\Re{\operatorname{Re}}
\def\Im{\operatorname{Im}}
\def\and{\quad\text{and}\quad}
\def\i{\text{\rm i}}
\def\hf{\widehat f}
\def\hu{\widehat u}
\def\tw{\widetilde w}
\def\tA{\widetilde A}
\def\tC{\widetilde C}
\def\tP{\widetilde P}
\def\tH{\widetilde H}
\def\si{\sigma}
\def\rd{\partial}
\def\esssup{\operatorname{ess.\, sup}}
\def\<{\left\langle}
\def\>{\right\rangle}
\def\bP{\mathbf P}
\def\bI{\mathbf I}
\def\mbA{\mathbf A}
\def\mbJ{\mathbf J}
\def\mbW{\mathbf W}
\def\bA{\mathbf A}
\def\bB{\mathbf B}
\def\bR{\mathbf R}
\def\bH{\mathbf H}
\def\bV{\mathbf V}
\def\bZ{\mathbf Z}
\def\bX{[H^1_0(\O)]^d}
\def\be{\mathbf e}
\def\br{\mathbf r}
\def\bu{\mathbf u}
\def\bv{\mathbf v}
\def\bw{\mathbf w}
\def\b1{\mathbf 1}
\def\bx{\mathbf x}
\def\bb{\mathbf b}
\def\bz{\mathbf z}
\def\bn{\mathbf n}

\def\Tau{{\mathcal T}}
\def\bPhi{{\boldsymbol \Phi}}
\def\bnu{{\boldsymbol \nu}}
\def\bphi{{\boldsymbol \phi}}
\def\bpsi{{\boldsymbol \psi}}
\def\bPi{{\boldsymbol \Pi}}
\def\Grad{\operatorname{grad}\,}
\def\Div{\operatorname{div}\,}
\def\Curl{\operatorname{curl}\,}
\def\grad{\nabla}
\def\div{\nabla\cdot}
\def\curl{\nabla\times}
\def\dim{\operatorname{dim}\,}

\def\mbe{\mathbf e}
\def\mbx{\mathbf x}
\def\mby{\mathbf y}
\def\dx{\kern0.1ex\operatorname{d\mbx}}
\def\dy{\kern0.1ex\operatorname{d\mby}}
\def\ds{\kern0.1ex\operatorname{ds}}
\def\dsig{\kern0.1ex \operatorname{d}\kern-0.5ex\boldsymbol{\sigma}}
\def\dhsig{\kern0.1ex \operatorname{d}\kern-0.5ex\hat{\boldsymbol{\sigma}}}
\def\dhatx{\kern0.1ex\operatorname{d\hat{\mbx}}}
\def\dhats{\kern0.1ex\operatorname{d\hat{s}}}
\def\mbF{\mathbf F}
\def\forany{\quad\forall}

\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\brknmH}[1]{{\vertiii {#1}}_H}
\newcommand{\brknmh}[1]{{\vertiii {#1}}_{h,K_{\delta,i}}}
\newcommand*{\avint}{\mathop{\ooalign{$\int$\cr$-$}}}

